Which One to Go: Security and Usability Evaluation of Mid-Air Gestures

With the emerging of touch-less human-computer interaction techniques and gadgets, mid-air hand gestures have been widely used for authentication. Much literature examined either the usability or security of a handful of gestures. This paper aims at quantifying usability and security of gestures as well as understanding their relationship across multiple gestures. To study gesture-based authentication, we design an authentication method that combines Dynamic Time Warping (DTW) and Support Vector Machine (SVM), and conducted a user study with 42 participants over a period of 6 weeks. We objectively quantify the usability of a gesture by the number of corners and the frame length of all gesture samples, quantify the security using the equal error rate (EER), and the consistency by EER over a period of time. Meanwhile, we obtain subjective evaluation of usability and security by conducting a survey. By examining the responses, we found that the subjective evaluation confirms with the objective ones, and usability is in inverse relationship with security. We studied the consistency of gestures and found that most participants forgot gestures to some degree and reinforcing the memorization of gestures is necessary to improve the authentication performance. Finally, we performed a study with another 17 participants on shoulder surfing attacks, where attackers can observe the victims multiple times. The results show that shoulder surfing does not help to boost the attacks.

==> Sections/appA.tex <==
% !Tex root = ../Midair_Gestures.tex
\section{Participant}
\label{sec:appA}

\begin{table}[h]
  \centering
  \scriptsize
  \vspace{-0mm} 
    \caption{Demographics and security preferences of the study participants.}
  \begin{tabular}{r|lll}
    \hline
    & \tabhead{\glab} & \tabhead{\gamazon} & \\  
      & n = 42 &  n = 61 & \\  \hline \hline
    Gender 	& 23.8\% & 47.5\% & Female \\
	 			& 76.2\% & 52.5\% & Male \\ \hline
	Age  		& 40.5\% & 3.3\% & 18 -- 24 \\
	 			& 54.7\% & 39.3\% & 25 -- 34 \\
	 			& 2.4\% & 27.9\% & 35 -- 44 \\ 
	 			& 2.4\% & 14.8\% & 45 -- 54 \\ 
	 			& 0\% & 14.7\% & 55 years or older \\  \hline
	Education	& 0\% & 1.6\% & No schooling completed \\
				& 2.4\% & 18.0\% & High school \\ 
				& 45.2\% & 60.7\% & College degree / Bachelor \\ 
				& 52.4\% & 19.6\% & Master / PhD Equivalent \\ \hline
	Occupation & 92.8\% & 3.3\% & Student \\
				& 4.8\% & 88.6\% & Employed \\
				& 2.4\% & 8.2\% & Unemployed/retired\\  \hline
	Current		& 2.4\% & 1.6\% & None \\
	preferred		& 78.6\% & 73.8\% & Digital PIN \\
	method 	& 73.8\% & 82.0\% & Alphanumeric password \\
     		& 21.4\% & 4.9\% & Token card \\
     				& 59.5\% & 41.5\% & Fingerprints \\
     				& 2.4\% & 11.5\% & Face recognition \\
   					& 9.5\% & 6.6\% & Graph / Android Pattern\\
    				& 0\% & 3.3\% & Other\\ \hline          
  \end{tabular}
  \label{tab:Demographics}
  \vspace{-0mm} 
\end{table} 


\begin{table}[h]
  \centering
  \scriptsize
  \vspace{-0mm} 
  \caption{Participants' responses to the acceptance to authentication system using mid-air gestures. 
   (A) responses to ``If it is available, I would like to use the mid-air gesture password to unlock (choose all that apply):''. (B) responses to ``How many times would you willing to use the mid-air gesture password in a week?''.}
  \begin{tabular}{r|lll}
    \hline
      &\tabhead{\glab} & \tabhead{\gamazon} & \\         
      & n = 42 &  n = 61 & \\  \hline \hline
            & 88.1\% & 70.5\% & Know depth sensors \\
            & 90.5\% & 65.5\% & Accept mid-air gesture\\ 
            &     &   & for game/computer operation \\ 
            & 68.9\% & 85.7\% & Accept mid-air gesture\\ 
            &  &        & for authentication \\
            
        \hline        
    (A)     & 2.4\% & 29.5\% & None \\
          & 52.4\% & 36.1\% & Phones/pads \\
            & 64.3\% & 54.1\% & Computers/laptops/devices \\
          & 33.3\% & 36.1\% & Physical doors \\
          & 7.1\% & 8.2\% & Bank accounts \\ 
          & 7.1\% & 16.4\% & Online accounts \\
          & 19.0\% & 23.0\% & Social network accounts \\ \hline
  
    (B) & 31.1\% & 14.3\% & 0 \\
          & 21.3\% & 16.7\% & 1 to 5 \\
            & 14.8\% & 38.1\% & 6 to 10 \\
          & 13.1\% & 9.5\% & 10 to 20 \\
          & 19.7\% & 21.4\% & more than 20 \\  \hline  
         
  \end{tabular}
  \vspace{-0mm} 
  \label{tab:acceptance}
\end{table}


==> Sections/appB.tex <==
% !Tex root = ../Midair_Gestures.tex
\section*{Appendix B}
\label{appB}



==> Sections/limitations.tex <==
\section{Limitations}
\label{related}

\xli{ There exists some limitations in our experiments. 1) The participants in \glab are heavily tech savvy since they were recruited in the universities with a good background of common authentication methods on mobile devices. 2) The results with respect to usability inferred in this paper need further validation by adding more samples. The sample of \glab seems a bit small for usability study and the sample of \gamazon didn't interact with our authentication system in practical. 3) The gestures were collected continuously without setting a resting interval for each participant, this may result in inference between two contiguous gesture types. 4) As shown in Table \ref{tab:data}, in the last week of gestures collection, we had a loss of about 60\% participants for follow up experiment. 
